Decompose, Optimize, and Reconstruct: Very Large Constant Multiplication at Scale

Efficient arithmetic circuit design for resourceconstrained hardware involves challenging combinatorial optimization problems, among which Multiple Constant Multiplication (MCM) is a prominent example. MCM aims at implementing multiplications by fixed integer constants using bit-shifts and additions/subtractions but optimal methods are typically limited to moderately-sized constants, e.g. 12 bits. For practical applications targeting larger precision, Very large Constant Multiplication (VLCM) is solved instead. Existing approaches typically address VLCM through a heuristic flow that decomposes large constants into patterns, applies MCM optimization techniques on moderately-sized targets, and reconstructs the final result. This paper proposes multiple improvements to this flow: new declarative optimization models for the pattern selection and for the reconstruction, as well as applying recent optimal MCM models. The cornerstones of the obtained improvements are (i) allowing the patterns to overlap, minimising the number of unique target constants for the MCM step and (ii) performing the reconstruction step optimally, instead of heuristically. In addition, we propose a globally-optimal VLCM approach and characterize its limits. We employ a mix of constraint programming and SAT to solve each step. Experimental results on synthetic and real-life signal processing and cryptographic benchmarks, with coefficient word lengths ranging from tens to thousands of bits, demonstrate that the proposed approach scales to very large precisions and consistently outperforms existing baselines.

==> abstract.tex <==
%Efficient arithmetic circuit design for resource-constrained hardware involves challenging combinatorial optimization problems, among which Multiple Constant Multiplication (MCM) is a prominent example.
%MCM aims at implementing multiplications by fixed integer constants using shift and addition/subtraction operations and has been extensively studied. 
%However, existing exact approaches (e.g. with SAT or Constraint Programming) achieve optimal or near-optimal solutions only for moderate-sized constants, typically up to 12 bits. 
%Hence, a typical methodology for dealing with larger constants is to subdivide them into smaller chunks, %perform 
%solve the MCM for small enough constants and reconstruct the Very Large Constant Multiplication (VLCM) result.
%This paper proposes a new efficient approach for the three-step design of VLCM.
%First, we improve the partitioning of multiple large constants into unique patterns by allowing them to overlap. 
%This new decomposition model reduces the number of unique patterns and allows us using optimal approaches for MCM in the second step. 
%Then, we provide several declarative optimization models for the optimal reconstruction step minimizing the number of necessary adders. 
%We test our approach on multiple synthetic and real-life benchmarks with constant word lengths going from tens to thousands of bits. 
%Experimental results show that our method scales to very large precisions and outperforms existing baselines in terms of number of adders.




==> fig/sat_patterns_fig.tex <==
\begin{figure}
\begin{tcolorbox}[ams align]
        \nonumber
        \varphi_1 :=& \, \left( \bigwedge_{m,w} \bigvee_{t,x} \gamma^{m,t}_{w,x} \right) \\
        \land& \, 
        \left( \bigwedge_{m,w,t_1,x_1} \bigwedge_{\substack{t_2,x_2: \\ t_2 \geq t_1, x_2 \geq x_1 \\ t_1 \neq t_2 \lor x_1 \neq x_2}} \neg \gamma^{m,t_1}_{w,x_1} \lor \neg \gamma^{m,t_2}_{w,x_2} \right) \\
        \varphi_2 := & \, 
        \left( \bigwedge_{m,t,x,w} \neg \gamma^{m,t}_{w,x} \lor \beta^t_x \right)
        \land
        \left( \bigwedge_{t,x} \neg \beta^t_x \lor \bigvee_{m,w} \gamma^{m,t}_{w,x} \right)\\
        \varphi_3 := & \, 
        \bigwedge_{m,t,x_1,w_1} \bigwedge_{\substack{x_2,w_2 \\ w_2 - w_1 \neq x_2 - x_1 \\ w_1 \leq w_2}} \neg \gamma^{m,t}_{w_1,x_1} \lor \neg \gamma^{m,t}_{w_2,x_2}\\
        \nonumber
        \varphi_4 := & \, 
        \left( \bigwedge_{t} \bigvee_{d} \delta^{d,t} \right) 
        \land \,
        \left( \bigwedge_{t,d,x} \alpha^d_x \lor \neg \beta^t_x \lor \neg \delta^{d,t} \right) \\
        \land & \,
        \left( \bigwedge_{t,d,x} \neg \alpha^d_x \lor \beta^t_x \lor \neg \delta^{d,t} \right) \\
        \varphi_5 := & \, 
        \left( \bigwedge_{m,t,x,w} \neg \gamma^{m,t}_{w,x} \lor \varepsilon^{m,t} \right)
        \land
        \left( \bigwedge_{\substack{t, m_1, m_2 \\ m_2 > m_1}} \neg \varepsilon^{m_1,t} \lor \neg \varepsilon^{m_2,t} \right) \\
        \varphi_6 := & \, 
        \bigwedge_{d} \alpha^d_0 .
\end{tcolorbox}
\caption{SAT formula for the pattern decomposition}
\label{fig:sat_patterns}
\end{figure}
